DictPFL: Efficient and Private Federated Learning on Encrypted Gradients

Federated Learning (FL) enables collaborative model training across institutions without sharing raw data. However, gradient sharing still risks privacy leakage, such as gradient inversion attacks. Homomorphic Encryption (HE) can secure aggregation but often incurs prohibitive computational and communication overhead. Existing HE-based FL methods sit at two extremes: encrypting all gradients for full privacy at high cost, or partially encrypting gradients to save resources while exposing vulnerabilities. We present DictPFL, a practical framework that achieves full gradient protection with minimal overhead. DictPFL encrypts every transmitted gradient while keeping non-transmitted parameters local, preserving privacy without heavy computation. It introduces two key modules: Decompose-for-Partial-Encrypt (DePE), which decomposes model weights into a static dictionary and an updatable lookup table, only the latter is encrypted and aggregated, while the static dictionary remains local and requires neither sharing nor encryption; and Prune-for-Minimum-Encrypt (PrME), which applies encryption-aware pruning to minimize encrypted parameters via consistent, history-guided masks. Experiments show that DictPFL reduces communication cost by 402-748$\times$ and accelerates training by 28-65$\times$ compared to fully encrypted FL, while outperforming state-of-the-art selective encryption methods by 51-155$\times$ in overhead and 4-19$\times$ in speed. Remarkably, DictPFL's runtime is within 2$\times$ of plaintext FL, demonstrating for the first time, that HE-based private federated learning is practical for real-world deployment. The code is publicly available at https://github.com/UCF-ML-Research/DictPFL.

==> tables/ablation_techs.tex <==
\begin{table}[h!]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{The results of different techniques of DicrPFL.}
\begin{tabular}{lcccccc}\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{10 Rounds} & \multicolumn{3}{c}{20 Rounds} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
 & Acc (\%) & Comm. & Time & Acc (\%) & Comm. & Time \\\midrule
FedHE-Full & 82.74 & 76.78 & 51.4 & 85.66 & 153.5 & 102 \\
FedLT & 82.79 & 6.235 & 14.3 & 85.61 & 12.47 & 28.5 \\
FedLT+TIP & 79.55 & 0.042 & 6.44 & 80.04 & 0.055 & 12.8 \\
FedLT+TIP+HRC & 82.67 & 0.103 & 6.42 & 85.58 & 0.122 & 12.8 \\\bottomrule
\end{tabular}
\label{t:ablation_techs}
\end{table}

==> tables/breakdown.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht!]
\renewcommand\arraystretch{0.9}
\centering
\scriptsize
\setlength{\tabcolsep}{8pt}
\caption{Detailed communication overhead and time breakdown for different operations for HE-based federated learning. DictPFL achieves excellent efficiency by significantly mitigating the bottlenecks. The experiments are performed under a homogenous 3-clients cross-silo setting on the GTSRB.}
\begin{tabular}{lcccccccc}\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Acc. (\%) $\uparrow$} & \multirow{2}{*}{Param. (M) $\downarrow$} & \multirow{2}{*}{Comm. (GB) $\downarrow$} & \multicolumn{5}{c}{Time $\downarrow$ } \\\cmidrule(lr){5-9}
 &  &  &  & Comm. (s) & Enc-Dec (s) & Client Train (s) & Server Agg. (s) & Total (min) \\\midrule
FedHE-Full & 92.57 & 1,717 & 153.6 & 1536 & 2875 & 71.83 & 815.8 & 88.32 \\
$\text{FedHE-FT}^{\text{Top2}}$ & 45.66 & 0.692 & 0.063 & 0.630 & 1.215 & 71.83 & 0.329 & 1.233 \\
FedML-HE & 92.57 & 5.733 & 16.42 & 164.2 & 295.5 & 71.83 & 85.27 & 10.28 \\
\rowcolor{Gray}
DictPFL (ours) & 97.60 & 2.867 & 0.256 & 2.566 & 4.717 & 71.83 & 1.342 & 1.340 \\\bottomrule
\label{t:breakdown}
\end{tabular}
\end{table*}

==> tables/different_dict.tex <==
\begin{table}[h!]
\centering
\small
\setlength{\tabcolsep}{8pt}
\caption{The results of DictPFL under different dictionary sizes $r$.}
\begin{tabular}{cccc}\toprule
$r$ & Accuracy (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ \\
 \midrule
2 & 74.26$_{\pm 0.5}$ & 0.046 & 6.11$_{\pm 0.1}$ \\
4 & 81.99$_{\pm 0.4}$ & 0.088 & 6.23$_{\pm 0.1}$ \\
8 & 82.67$_{\pm 0.2}$ & 0.160 & 6.42$_{\pm 0.2}$ \\
16 & 82.71$_{\pm 0.2}$ & 0.332 & 7.27$_{\pm 0.1}$ \\\bottomrule
\end{tabular}
\label{t:different_dicts}
\end{table}

==> tables/different_tau.tex <==
% \begin{table}[h!]
% \renewcommand\arraystretch{0.9}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{7pt}
% \caption{The results of DictPFL under different pruning patience $\tau$. The ``non" denotes the results without pruning.}
% \begin{tabular}{ccccccc}\toprule
% \multirow{2}{*}{$\tau$} & \multicolumn{3}{c}{10 Rounds} & \multicolumn{3}{c}{20 Rounds} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
%  & Acc. (\%) & Comm. & Time & Acc (\%) & Comm. & Time \\\midrule
% 3 & 82.29 & 0.003 & 6.36 & 85.02 & 0.005 & 12.72 \\
% 5 & 82.67 & 0.103 & 6.42 & 85.58 & 0.151 & 12.81 \\
% 10 & 82.77 & 0.474 & 6.63 & 85.72 & 1.185 & 13.40 \\\midrule
% non & 82.79 & 6.235 & 14.3 & 85.61 & 12.47 & 28.47 \\\bottomrule
% \end{tabular}
% \label{t:tau}
% \end{table}


\begin{table}[h!]
\renewcommand\arraystretch{0.9}
\centering
\small
\setlength{\tabcolsep}{7pt}
\caption{Various pruning patiences under \(s\%=70\%\) and \(\beta=0.2\).}
\begin{tabular}{cccc}\toprule
$\tau$ & Accuracy (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ \\\midrule
1 & 80.55$_{\pm 0.6}$ & 0.001 & 6.26$_{\pm 0.1}$\\
3 & 82.29$_{\pm 0.3}$ & 0.003 & 6.36$_{\pm 0.1}$\\
5 & 82.67$_{\pm 0.2}$ & 0.160 & 6.42$_{\pm 0.2}$ \\
10 & 82.77$_{\pm 0.3}$ & 0.474 & 6.92$_{\pm 0.1}$ \\\bottomrule
\end{tabular}
\label{t:tau}
\end{table}




==> tables/main_results.tex <==
% \begin{table*}[ht!]
% \renewcommand\arraystretch{0.9}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.5pt}
% \caption{End-to-end comparison on the ViT model across various datasets in a three-client cross-silo federated learning setting. ``Homo" indicates homogeneous datasets, while ``Heter" represents heterogeneous datasets characterized by a Dirichlet distribution with $\alpha = 0.3$. The rounds are set to \{$5$, $10$, $20$\} and \{$10$, $15$, $30$\} for homogeneous and heterogeneous settings, respectively.}
% \begin{tabular}{llcccccccccccc}\toprule
%  & \multicolumn{1}{l}{\multirow{2}{*}{Methods}} & \multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{Diabetic Retinopathy} & \multicolumn{3}{c}{GTSRB} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% &  & Acc. (\%) $\uparrow$  & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ & Acc. (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ & Acc. (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ \\\midrule
% \multirow{4}{*}{\cellcolor{white}Homo} & FedHE-Full & 98.02 & 38.39 & 24.3 & 82.74 & 76.78 & 51.4 & 92.57 & 1536 & 88.3 \\
% & $\text{FedHE-FT}^{\text{Top2}}$ & 94.68 & 0.004 & 1.54 & 75.17 & 0.006 & 6.36 & 45.66 & 0.063 & 1.25 \\
% % & FedHE-Lora & 97.41 & 5.056 & 1909 & 82.53 & 7.492 & 2382 &  &  &  &  \\
% & FedML-HE & 97.73 & 3.840 & 3.81 & 81.02 & 7.675 & 10.9 & 91.88 & 15.36 & 9.91\\
% \rowcolor{Gray}
% \cellcolor{white} & DictPFL (ours) & 97.94 &  0.095 & 1.59 & 82.67 & 0.103 & 6.42 & 97.60 & 0.257 & 1.34 \\\midrule
% \multirow{4}{*}{Heter} & FedHE-Full & 98.09 & 76.78 & 46.1 & 80.90 & 115.2 & 70.3 & 92.15 & 230.4 & 114  \\
% & $\text{FedHE-FT}^{\text{Top2}}$ & 94.64 & 0.009 & 3.09 & 73.66 & 0.007 & 9.55 & 37.88 & 0.094 & 1.85 \\
% % & FedHE-Lora & 97.62 & 2.528 & 3436 & 81.72 & 11.23 & 3574 &  &  &  \\
% & FedML-HE & 98.02 & 7.679 & 10.4 & 80.55 & 11.52 & 15.6 & 92.23 & 23.04 & 13.0 \\
% \rowcolor{Gray}
% \cellcolor{white} & DictPFL (ours) & 97.77 & 0.115 & 3.15 & 81.45 & 0.145 & 9.62 & 96.06 & 0.318 & 1.97 \\\bottomrule
% \end{tabular}
% \label{tab:main_results}
% \end{table*}



\begin{table*}[ht!]
\renewcommand\arraystretch{0.9}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{End-to-end comparison on the ViT model across various datasets in a three-client cross-silo federated learning setting. ``Homo" indicates homogeneous datasets, while ``Heter" represents heterogeneous datasets characterized by a Dirichlet distribution with $\alpha = 0.3$. The rounds are set to \{$5$, $10$, $20$\} and \{$10$, $15$, $30$\} for homogeneous and heterogeneous settings, respectively.}
\begin{tabular}{llcccccccccccc}\toprule
 & \multicolumn{1}{l}{\multirow{2}{*}{Methods}} & \multicolumn{3}{c}{ViT-GTSRB} & \multicolumn{3}{c}{BERT-AgNews} & \multicolumn{3}{c}{TinyLlama-MetaMathQA} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
&  & Acc. (\%) $\uparrow$  & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ & Acc. (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (min) $\downarrow$ & Acc. (\%) $\uparrow$ & Comm. (TB) $\downarrow$ & Time (hour) $\downarrow$ \\\midrule
\multirow{4}{*}{\cellcolor{white}Homo} & FedHE-Full & 92.57 & 1536 & 88.30 & 91.38 & 137.22 & 57.1 & 45.86 & 30.03 & 214.2 \\
& $\text{FedHE-FT}^{\text{Top2}}$ & 45.66 & 0.06 & 1.25 & 90.05 & 17.48 & 7.3 & 6.92 & 2.40 & 17.9 \\
& FedML-HE & 91.88 & 15.36 & 9.91 & 91.38 & 13.71 & 5.8 & 45.86 & 3.00 & 22.6\\
\rowcolor{Gray}
\cellcolor{white} & DictPFL (ours) & 90.32 & 9.81 & 4.26 & 42.23 & 0.79 & 6.5 & 97.60 & 0.257 & 1.34 \\\midrule
\multirow{4}{*}{Heter} & FedHE-Full & 92.15 & 230.4 & 114 & 90.74 & 205.80 & 85.6 & 42.05 & 43.68 & 310.9 \\
& $\text{FedHE-FT}^{\text{Top2}}$ & 37.88 & 0.09 & 1.85 & 90.02 & 24.09 & 10.0 & 6.43 & 2.46 & 18.2\\
& FedML-HE & 92.23 & 23.04 & 13.00 & 90.74 & 20.58 & 8.8 & 42.05 & 4.37 & 32.3 \\
\rowcolor{Gray}
\cellcolor{white} & DictPFL (ours) & 96.06 & 0.32 & 1.97 & 90.15 & 11.38 & 5.0 & 40.74 & 0.82 & 6.8 \\\bottomrule
\end{tabular}
\label{tab:main_results}
\end{table*}







==> tables/methods.tex <==
% \begin{table}[t!]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{8pt}
% \caption{Comparison of various HE-based federated learning against three key criteria: Privacy, Utility, and Efficiency.}
% \begin{tabular}{lccc}\toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Criteria} \\\cmidrule(lr){2-4}
%  & Privacy -- \ref{c:1} & Utility -- \ref{c:2} & Efficiency -- \ref{c:3} \\\midrule
% FedHE-Full & \ding{51} & \ding{51} & \ding{55} \\
% $\text{FedHE-FT}^{\text{Top2}}$ & \ding{51} & \ding{55} & \ding{51} \\
% FedML-HE~\cite{du2023hefed1} & \ding{55} & \ding{51} & \ding{55} \\
% \rowcolor{Gray}
% DictPFL (ours) & \ding{51} & \ding{51} & \ding{51} \\\bottomrule
% \end{tabular}
% \label{tab:methods_criteria}
% \end{table}

==> tables/models.tex <==
\begin{table}[h!]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{DictPFL's performance on different models. The values in the brackets are FedHE-ML with 10\% encryption ratio.}
\begin{tabular}{lcccc}\toprule
Model & Acc. (\%) $\uparrow$ & Comm. (GB) $\downarrow$ & Time (mins) $\downarrow$ & Attack Score $\downarrow$ \\\midrule
DeiT & 80.90 & 0.082 (5.85) & 3.10 (7.38) & 0.0 (0.83)\\
Swin & 80.22 & 0.066 (4.57) & 2.46 (6.47) & 0.0 (0.79)\\
ViT & 82.67 & 0.103 (7.68) & 6.42 (10.9) & 0.0 (0.88) \\\bottomrule
\label{t:models}
\end{tabular}
\end{table}
